Can the violent merger of white dwarfs explain the slowest declining Type Ia supernova SN 2011aa?

We present optical observations and Monte Carlo radiative transfer modeling of the Type Ia supernova SN 2011aa. With a $\Delta m_{15} (B)$ of $0.59 \pm 0.07$ mag and a peak magnitude $M_{\rm B}$ of $-19.30 \pm 0.27$ mag, SN 2011aa has the slowest decline rate among SNe Ia. The secondary maximum in the $I$-band is absent or equally bright as the primary maximum. The velocity of C II is lower than the velocity of Si II. This indicates either presence of C at lower velocities than Si or a line of sight effect. Application of Arnett's radiation diffusion model to the bolometric light curve indicates a massive ejecta $M_{\rm{ej}} ~ 1.8 - 2.6~M_{\odot}$. The slow decline rate and large ejecta mass, with a normal peak magnitude, are well explained by double degenerate, violent merger explosion model. The synthetic spectra and light curves generated with SEDONA considering a violent merger density profile match the observations.

==> Model_comp.tex <==
\begin{table*}
\centering
\caption{\texttt{SEDONA} model features}
\label{tab:Models}
\begin{tabular}{lcccccc}
\hline\hline
Model Name & Density$^{*}$   &    Abundance    &  $\epsilon$  & $\Delta m_{15} (B)$ (mag) & $M_{\rm B}$ (mag)  & $^{56}$Ni ($M_{\odot}$)\\
\hline\hline  
Model 1  & violent merger &  violent merger & 1.0    &  0.96  & $-$19.20 & 0.62 \\
Model 2  & violent merger &  modified abundance &  1.0    &  0.96  & $-$19.39 & 0.68 \\
         &                &  $+$ increased $^{56}$Ni &    &  &    &  \\
Model 3  & violent merger &  same as Model 2 & 0.5    & 0.77  & $-$19.35  & 0.68 \\
Model 4  & violent merger & same as Model 2 & 0.3   & 0.59   & $-$19.31  & 0.68 \\
\hline
\multicolumn{2}{l}{$^{*}$\footnotesize{One dimensional density of the violent merger model}.}
\end{tabular}
\end{table*}

==> optical_phot.tex <==
\afterpage{
\begin{longtable}[hbt!]{cccccc}
\caption{$UBVRI$ magnitudes of SN~2011aa} \label{tab:uvphotlog} \\

\hline \multicolumn{1}{c}{JD} & \multicolumn{1}{c}{Phase$^*$} & \multicolumn{1}{c}{Filter} & \multicolumn{1}{c}{Magnitude (mag)} & \multicolumn{1}{c}{Error (mag)} \\ \hline 
\endfirsthead

\multicolumn{6}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{c}{JD} & \multicolumn{1}{c}{Phase$^*$} & \multicolumn{1}{c}{Filter} & \multicolumn{1}{c}{Magnitude (mag)} & \multicolumn{1}{c}{Error (mag)} \\ \hline 
\endhead

\hline \multicolumn{5}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot
2455601.327 & -10.191 &      B & 15.248 & 0.012 \\
2455602.413 &  -9.118 &      B & 15.121 & 0.013 \\
2455603.352 &  -8.192 &      B & 15.027 & 0.009 \\
2455604.220 &  -7.335 &      B & 14.962 & 0.008 \\
2455609.156 &  -2.462 &      B & 14.723 & 0.038 \\
2455610.188 &  -1.443 &      B & 14.757 & 0.063 \\
2455612.131 &   0.475 &      B & 14.718 & 0.011 \\
2455613.125 &   1.456 &      B & 14.719 & 0.010 \\
2455614.072 &   2.391 &      B & 14.734 & 0.007 \\
2455615.188 &   3.493 &      B & 14.717 & 0.014 \\
2455618.190 &   6.456 &      B & 14.829 & 0.015 \\
2455620.103 &   8.345 &      B & 14.876 & 0.008 \\
2455621.072 &   9.301 &      B & 14.930 & 0.020 \\
2455622.097 &  10.313 &      B & 14.987 & 0.008 \\
2455626.431 &  14.591 &      B & 15.292 & 0.023 \\
2455627.069 &  15.221 &      B & 15.362 & 0.023 \\
2455628.069 &  16.208 &      B & 15.415 & 0.019 \\
2455629.090 &  17.216 &      B & 15.504 & 0.015 \\
2455635.234 &  23.281 &      B & 15.987 & 0.022 \\
2455636.179 &  24.214 &      B & 16.057 & 0.011 \\
2455637.133 &  25.156 &      B & 16.119 & 0.017 \\
2455639.208 &  27.204 &      B & 16.208 & 0.040 \\
2455642.090 &  30.049 &      B & 16.379 & 0.011 \\
2455643.077 &  31.024 &      B & 16.418 & 0.022 \\
2455646.161 &  34.068 &      B & 16.526 & 0.008 \\
2455649.167 &  37.036 &      B & 16.611 & 0.011 \\
2455653.198 &  41.015 &      B & 16.709 & 0.014 \\
2455655.264 &  43.054 &      B & 16.777 & 0.006 \\
2455662.090 &  49.793 &      B & 16.961 & 0.011 \\
2455667.243 &  54.880 &      B & 17.086 & 0.020 \\
2455672.280 &  59.852 &      B & 17.232 & 0.018 \\
2455681.221 &  68.678 &      B & 17.504 & 0.008 \\
2455685.164 &  72.571 &      B & 17.619 & 0.009 \\
2455694.115 &  81.407 &      B & 17.918 & 0.012 \\
2455709.159 &  96.258 &      B & 18.435 & 0.010 \\
2455601.327 & -10.191 &      I & 15.236 & 0.006 \\
2455602.413 &  -9.118 &      I & 15.147 & 0.015 \\
2455603.352 &  -8.192 &      I & 15.065 & 0.014 \\
2455604.220 &  -7.335 &      I & 15.020 & 0.010 \\
2455609.156 &  -2.462 &      I & 14.815 & 0.015 \\
2455610.188 &  -1.443 &      I & 14.787 & 0.013 \\
2455612.131 &   0.475 &      I & 14.749 & 0.010 \\
2455613.125 &   1.456 &      I & 14.742 & 0.012 \\
2455614.072 &   2.391 &      I & 14.733 & 0.006 \\
2455615.188 &   3.493 &      I & 14.715 & 0.015 \\
2455618.190 &   6.456 &      I & 14.698 & 0.015 \\
2455620.103 &   8.345 &      I & 14.692 & 0.009 \\
2455621.072 &   9.301 &      I & 14.731 & 0.032 \\
2455622.097 &  10.313 &      I & 14.733 & 0.016 \\
2455626.431 &  14.591 &      I & 14.789 & 0.022 \\
2455627.069 &  15.221 &      I & 14.770 & 0.030 \\
2455628.069 &  16.208 &      I & 14.761 & 0.012 \\
2455629.090 &  17.216 &      I & 14.775 & 0.022 \\
2455635.234 &  23.281 &      I & 14.803 & 0.013 \\
2455636.179 &  24.214 &      I & 14.799 & 0.019 \\
2455637.133 &  25.156 &      I & 14.802 & 0.041 \\
2455639.208 &  27.204 &      I & 14.778 & 0.024 \\
2455642.090 &  30.049 &      I & 14.841 & 0.013 \\
2455643.077 &  31.024 &      I & 14.866 & 0.024 \\
2455646.161 &  34.068 &      I & 14.924 & 0.011 \\
2455649.167 &  37.036 &      I & 14.944 & 0.022 \\
2455653.198 &  41.015 &      I & 15.066 & 0.009 \\
2455655.264 &  43.054 &      I & 15.135 & 0.011 \\
2455662.090 &  49.793 &      I & 15.379 & 0.011 \\
2455667.243 &  54.880 &      I & 15.658 & 0.019 \\
2455672.280 &  59.852 &      I & 15.793 & 0.019 \\
2455681.221 &  68.678 &      I & 16.201 & 0.017 \\
2455685.164 &  72.571 &      I & 16.401 & 0.017 \\
2455694.115 &  81.407 &      I & 16.833 & 0.018 \\
2455701.095 &  88.297 &      I & 17.089 & 0.014 \\
2455726.122 & 113.003 &      I & 18.398 & 0.032 \\
2455601.327 & -10.191 &      R & 15.229 & 0.011 \\
2455602.413 &  -9.118 &      R & 15.117 & 0.012 \\
2455603.352 &  -8.192 &      R & 15.036 & 0.013 \\
2455604.220 &  -7.335 &      R & 14.987 & 0.007 \\
2455609.156 &  -2.462 &      R & 14.730 & 0.008 \\
2455610.188 &  -1.443 &      R & 14.703 & 0.015 \\
2455612.131 &   0.475 &      R & 14.675 & 0.013 \\
2455613.125 &   1.456 &      R & 14.663 & 0.006 \\
2455614.072 &   2.391 &      R & 14.658 & 0.009 \\
2455615.188 &   3.493 &      R & 14.625 & 0.010 \\
2455618.190 &   6.456 &      R & 14.665 & 0.014 \\
2455620.103 &   8.345 &      R & 14.678 & 0.005 \\
2455621.072 &   9.301 &      R & 14.696 & 0.020 \\
2455622.097 &  10.313 &      R & 14.729 & 0.019 \\
2455626.431 &  14.591 &      R & 14.852 & 0.029 \\
2455627.069 &  15.221 &      R & 14.825 & 0.022 \\
2455628.069 &  16.208 &      R & 14.846 & 0.008 \\
2455629.090 &  17.216 &      R & 14.862 & 0.020 \\
2455635.234 &  23.281 &      R & 15.014 & 0.020 \\
2455636.179 &  24.214 &      R & 15.033 & 0.016 \\
2455637.133 &  25.156 &      R & 15.050 & 0.023 \\
2455639.208 &  27.204 &      R & 15.112 & 0.020 \\
2455642.090 &  30.049 &      R & 15.131 & 0.010 \\
2455643.077 &  31.024 &      R & 15.162 & 0.023 \\
2455646.161 &  34.068 &      R & 15.223 & 0.008 \\
2455649.167 &  37.036 &      R & 15.288 & 0.013 \\
2455653.198 &  41.015 &      R & 15.420 & 0.011 \\
2455655.264 &  43.054 &      R & 15.478 & 0.007 \\
2455662.090 &  49.793 &      R & 15.744 & 0.018 \\
2455667.243 &  54.880 &      R & 15.961 & 0.011 \\
2455672.280 &  59.852 &      R & 16.167 & 0.025 \\
2455681.221 &  68.678 &      R & 16.575 & 0.008 \\
2455685.164 &  72.571 &      R & 16.751 & 0.018 \\
2455694.115 &  81.407 &      R & 17.160 & 0.017 \\
2455701.095 &  88.297 &      R & 17.495 & 0.012 \\
2455709.159 &  96.258 &      R & 17.828 & 0.021 \\
2455726.122 & 113.003 &      R & 18.619 & 0.032 \\
2455740.126 & 126.827 &      R & 19.370 & 0.019 \\
2455601.327 & -10.191 &      U & 14.696 & 0.033 \\
2455602.413 &  -9.118 &      U & 14.549 & 0.069 \\
2455603.352 &  -8.192 &      U & 14.478 & 0.016 \\
2455604.220 &  -7.335 &      U & 14.415 & 0.032 \\
2455610.188 &  -1.443 &      U & 14.201 & 0.069 \\
2455612.131 &   0.475 &      U & 14.197 & 0.041 \\
2455613.125 &   1.456 &      U & 14.227 & 0.045 \\
2455614.072 &   2.391 &      U & 14.203 & 0.036 \\
2455615.188 &   3.493 &      U & 14.239 & 0.030 \\
2455618.190 &   6.456 &      U & 14.364 & 0.013 \\
2455620.103 &   8.345 &      U & 14.432 & 0.011 \\
2455621.072 &   9.301 &      U & 14.533 & 0.053 \\
2455622.097 &  10.313 &      U & 14.589 & 0.021 \\
2455627.069 &  15.221 &      U & 15.054 & 0.024 \\
2455628.069 &  16.208 &      U & 15.143 & 0.041 \\
2455629.090 &  17.216 &      U & 15.218 & 0.012 \\
2455635.234 &  23.281 &      U & 15.816 & 0.023 \\
2455636.179 &  24.214 &      U & 15.926 & 0.043 \\
2455637.133 &  25.156 &      U & 15.922 & 0.035 \\
2455639.208 &  27.204 &      U & 16.076 & 0.069 \\
2455642.090 &  30.049 &      U & 16.260 & 0.033 \\
2455643.077 &  31.024 &      U & 16.313 & 0.021 \\
2455646.161 &  34.068 &      U & 16.435 & 0.019 \\
2455649.167 &  37.036 &      U & 16.541 & 0.046 \\
2455655.264 &  43.054 &      U & 16.673 & 0.017 \\
2455662.090 &  49.793 &      U & 16.884 & 0.025 \\
2455672.280 &  59.852 &      U & 17.092 & 0.036 \\
2455685.164 &  72.571 &      U & 17.486 & 0.024 \\
2455601.327 & -10.191 &      V & 15.298 & 0.017 \\
2455602.413 &  -9.118 &      V & 15.163 & 0.018 \\
2455603.352 &  -8.192 &      V & 15.075 & 0.011 \\
2455604.220 &  -7.335 &      V & 15.010 & 0.016 \\
2455609.156 &  -2.462 &      V & 14.756 & 0.008 \\
2455610.188 &  -1.443 &      V & 14.743 & 0.018 \\
2455612.131 &   0.475 &      V & 14.708 & 0.010 \\
2455613.125 &   1.456 &      V & 14.688 & 0.010 \\
2455614.072 &   2.391 &      V & 14.686 & 0.005 \\
2455615.188 &   3.493 &      V & 14.666 & 0.023 \\
2455618.190 &   6.456 &      V & 14.705 & 0.019 \\
2455620.103 &   8.345 &      V & 14.728 & 0.004 \\
2455621.072 &   9.301 &      V & 14.742 & 0.018 \\
2455622.097 &  10.313 &      V & 14.788 & 0.017 \\
2455626.431 &  14.591 &      V & 14.944 & 0.028 \\
2455627.069 &  15.221 &      V & 14.969 & 0.027 \\
2455628.069 &  16.208 &      V & 15.019 & 0.013 \\
2455629.090 &  17.216 &      V & 15.050 & 0.014 \\
2455635.234 &  23.281 &      V & 15.284 & 0.012 \\
2455636.179 &  24.214 &      V & 15.320 & 0.022 \\
2455637.133 &  25.156 &      V & 15.344 & 0.021 \\
2455639.208 &  27.204 &      V & 15.430 & 0.024 \\
2455642.090 &  30.049 &      V & 15.478 & 0.009 \\
2455643.077 &  31.024 &      V & 15.508 & 0.015 \\
2455646.161 &  34.068 &      V & 15.605 & 0.012 \\
2455649.167 &  37.036 &      V & 15.712 & 0.010 \\
2455653.198 &  41.015 &      V & 15.795 & 0.011 \\
2455655.264 &  43.054 &      V & 15.852 & 0.012 \\
2455662.090 &  49.793 &      V & 16.080 & 0.018 \\
2455667.243 &  54.880 &      V & 16.239 & 0.017 \\
2455672.280 &  59.852 &      V & 16.411 & 0.021 \\
2455681.221 &  68.678 &      V & 16.760 & 0.008 \\
2455685.164 &  72.571 &      V & 16.919 & 0.021 \\
2455694.115 &  81.407 &      V & 17.275 & 0.012 \\
2455701.095 &  88.297 &      V & 17.557 & 0.009 \\
2455709.159 &  96.258 &      V & 17.890 & 0.019 \\
2455726.122 & 113.003 &      V & 18.616 & 0.029 \\
2455740.126 & 126.827 &      V & 19.230 & 0.025 \\
\hline
\multicolumn{2}{l}{$^*$\footnotesize{Rest frame time since $B$-band maximum (2455611.65)}.}
\end{longtable}
}

==> spectral_log.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{3pt}
\caption{Log of spectroscopic observations of SN~2011aa from HCT.}
\label{tab:speclog}
\begin{tabular}{c c c c}
\hline \hline
    JD &     Date &  Phase* & Range  \\
 &   &  (d)    & (\AA)         \\
 \hline \noalign{\smallskip}    
 2011/02/08 &  2455601.36  &     -10.16 & 3500-7800; 5200-9100 \\
 2011/02/09 &  2455602.16  &     -9.37  & 3500-7800; 5200-9100 \\
 2011/02/10 &  2455603.37  &     -8.17  & 3500-7800; 5200-9100 \\
 2011/02/11 &  2455604.39  &     -7.17  & 3500-7800; 5200-9100 \\
 2011/02/17 &  2455610.22  &     -1.41  & 3500-7800; 5200-9100 \\
 2011/02/19 &  2455612.15  &      0.49  & 3500-7800; 5200-9100 \\
 2011/02/20 &  2455613.34  &      1.67  & 3500-7800; 5200-9100 \\
 2011/02/21 &  2455614.17  &      2.49  & 3500-7800; 5200-9100 \\
 2011/02/22 &  2455615.22  &      3.52  & 3500-7800; 5200-9100 \\
 2011/02/28 &  2455621.10  &      9.33  & 3500-7800; 5200-9100 \\
 2011/03/01 &  2455622.14  &     10.36  & 3500-7800; 5200-9100 \\
 2011/03/07 &  2455628.10  &     16.24  & 3500-7800; 5200-9100 \\
 2011/03/08 &  2455629.13  &     17.26  & 3500-7800; 5200-9100 \\
 2011/03/15 &  2455636.20  &     24.23  & 3500-7800; 5200-9100 \\
 2011/03/16 &  2455637.17  &     25.19  & 3500-7800; 5200-9100 \\
 2011/03/21 &  2455642.13  &     30.09  & 3500-7800; 5200-9100 \\
 2011/03/23 &  2455644.07  &     32.0   & 3500-7800; 5200-9100 \\
 2011/03/25 &  2455646.31  &     34.22  & 3500-7800; 5200-9100 \\
 2011/04/01 &  2455653.30  &     41.12  & 3500-7800; 5200-9100 \\
 2011/04/10 &  2455662.12  &     49.82  & 3500-7800; 5200-9100 \\
 2011/04/15 &  2455667.21  &     54.85  & 3500-7800; 5200-9100 \\
 2011/04/20 &  2455672.20  &     59.77  & 3500-7800; 5200-9100 \\
 2011/04/29 &  2455681.18  &     68.64  & 3500-7800; 5200-9100 \\
 

\noalign{\smallskip} \hline
\multicolumn{3}{l}{$^*$\footnotesize{Rest frame time since $B$-band maximum (2455611.65).}}
\end{tabular}
\end{table}


==> uvopt_phot.tex <==
\afterpage{
\begin{longtable}[hbt!]{cccccc}
\caption{$Swift$-UVOT magnitudes of SN~2011aa} \label{tab:uvphotlog} \\

\hline \multicolumn{1}{c}{JD} & \multicolumn{1}{c}{Phase$^*$} & \multicolumn{1}{c}{Filter} & \multicolumn{1}{c}{Magnitude (mag)} & \multicolumn{1}{c}{Error (mag)} \\ \hline 
\endfirsthead

\multicolumn{6}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{c}{JD} & \multicolumn{1}{c}{Phase$^*$} & \multicolumn{1}{c}{Filter} & \multicolumn{1}{c}{Magnitude (mag)} & \multicolumn{1}{c}{Error (mag)} \\ \hline 
\endhead

\hline \multicolumn{5}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot
2455603.66 &  -7.89 &    uvb & 15.00 &  0.02 \\
2455605.91 &  -5.67 &    uvb & 14.91 &  0.03 \\
2455607.08 &  -4.51 &    uvb & 14.87 &  0.04 \\
2455609.95 &  -1.68 &    uvb & 14.85 &  0.04 \\
2455611.23 &  -0.41 &    uvb & 14.75 &  0.04 \\
2455613.63 &   1.95 &    uvb & 14.81 &  0.04 \\
2455615.07 &   3.38 &    uvb & 14.82 &  0.04 \\
2455617.54 &   5.81 &    uvb & 14.88 &  0.04 \\
2455621.56 &   9.78 &    uvb & 15.01 &  0.04 \\
2455632.90 &  20.98 &    uvb & 15.82 &  0.04 \\
2455635.07 &  23.12 &    uvb & 15.99 &  0.04 \\
2455637.27 &  25.29 &    uvb & 16.26 &  0.06 \\
2455640.25 &  28.23 &    uvb & 16.29 &  0.06 \\
2455649.14 &  37.01 &    uvb & 16.50 &  0.06 \\
2455657.70 &  45.46 &    uvb & 16.71 &  0.08 \\
2455603.66 &  -7.89 &   uvm2 & 15.83 &  0.03 \\
2455605.91 &  -5.67 &   uvm2 & 15.72 &  0.05 \\
2455607.08 &  -4.51 &   uvm2 & 15.69 &  0.05 \\
2455609.95 &  -1.68 &   uvm2 & 15.98 &  0.05 \\
2455611.23 &  -0.41 &   uvm2 & 15.79 &  0.05 \\
2455613.63 &   1.95 &   uvm2 & 15.95 &  0.05 \\
2455615.07 &   3.38 &   uvm2 & 16.10 &  0.06 \\
2455617.54 &   5.81 &   uvm2 & 16.24 &  0.06 \\
2455621.56 &   9.78 &   uvm2 & 16.69 &  0.07 \\
2455632.90 &  20.98 &   uvm2 & 18.27 &  0.15 \\
2455635.07 &  23.12 &   uvm2 & 18.60 &  0.22 \\
2455637.27 &  25.29 &   uvm2 & 18.97 &  0.24 \\
2455640.25 &  28.23 &   uvm2 & 18.60 &  0.19 \\
2455649.14 &  37.01 &   uvm2 & 18.60 &  0.16 \\
2455657.70 &  45.46 &   uvm2 & 18.45 &  0.15 \\
2455603.66 &  -7.89 &    uvu & 14.23 &  0.04 \\
2455605.91 &  -5.67 &    uvu & 14.14 &  0.04 \\
2455607.08 &  -4.51 &    uvu & 14.10 &  0.03 \\
2455609.95 &  -1.68 &    uvu & 14.27 &  0.04 \\
2455611.23 &  -0.41 &    uvu & 14.16 &  0.04 \\
2455613.63 &   1.95 &    uvu & 14.27 &  0.04 \\
2455615.07 &   3.38 &    uvu & 14.26 &  0.04 \\
2455617.54 &   5.81 &    uvu & 14.38 &  0.04 \\
2455621.56 &   9.78 &    uvu & 14.59 &  0.04 \\
2455632.90 &  20.98 &    uvu & 15.86 &  0.06 \\
2455635.07 &  23.12 &    uvu & 15.94 &  0.06 \\
2455637.27 &  25.29 &    uvu & 16.17 &  0.04 \\
2455640.25 &  28.23 &    uvu & 16.38 &  0.08 \\
2455649.14 &  37.01 &    uvu & 16.54 &  0.08 \\
2455657.70 &  45.46 &    uvu & 16.96 &  0.12 \\
2455603.66 &  -7.89 &    uvv & 14.99 &  0.04 \\
2455605.91 &  -5.67 &    uvv & 14.86 &  0.03 \\
2455607.08 &  -4.51 &    uvv & 14.85 &  0.04 \\
2455609.95 &  -1.68 &    uvv & 14.85 &  0.04 \\
2455611.23 &  -0.41 &    uvv & 14.69 &  0.04 \\
2455613.63 &   1.95 &    uvv & 14.68 &  0.04 \\
2455615.07 &   3.38 &    uvv & 14.67 &  0.05 \\
2455617.54 &   5.81 &    uvv & 14.67 &  0.05 \\
2455621.56 &   9.78 &    uvv & 14.72 &  0.05 \\
2455632.90 &  20.98 &    uvv & 15.18 &  0.06 \\
2455635.07 &  23.12 &    uvv & 15.25 &  0.05 \\
2455637.27 &  25.29 &    uvv & 15.44 &  0.05 \\
2455640.25 &  28.23 &    uvv & 15.59 &  0.07 \\
2455649.14 &  37.01 &    uvv & 15.54 &  0.06 \\
2455657.70 &  45.46 &    uvv & 15.79 &  0.08 \\
2455603.66 &  -7.89 &   uvw1 & 15.10 &  0.04 \\
2455605.91 &  -5.67 &   uvw1 & 15.05 &  0.04 \\
2455607.08 &  -4.51 &   uvw1 & 14.99 &  0.04 \\
2455609.95 &  -1.68 &   uvw1 & 15.20 &  0.04 \\
2455611.23 &  -0.41 &   uvw1 & 15.04 &  0.04 \\
2455613.63 &   1.95 &   uvw1 & 15.17 &  0.04 \\
2455615.07 &   3.38 &   uvw1 & 15.23 &  0.05 \\
2455617.54 &   5.81 &   uvw1 & 15.46 &  0.06 \\
2455621.56 &   9.78 &   uvw1 & 15.76 &  0.05 \\
2455632.90 &  20.98 &   uvw1 & 17.29 &  0.11 \\
2455635.07 &  23.12 &   uvw1 & 17.38 &  0.11 \\
2455637.27 &  25.29 &   uvw1 & 17.59 &  0.11 \\
2455640.25 &  28.23 &   uvw1 & 17.65 &  0.15 \\
2455649.14 &  37.01 &   uvw1 & 17.63 &  0.11 \\
2455657.70 &  45.46 &   uvw1 & 17.92 &  0.15 \\
2455603.66 &  -7.89 &   uvw2 & 16.20 &  0.05 \\
2455605.91 &  -5.67 &   uvw2 & 16.22 &  0.05 \\
2455607.08 &  -4.51 &   uvw2 & 16.13 &  0.05 \\
2455609.95 &  -1.68 &   uvw2 & 16.39 &  0.05 \\
2455611.23 &  -0.41 &   uvw2 & 16.19 &  0.05 \\
2455613.63 &   1.95 &   uvw2 & 16.37 &  0.06 \\
2455615.07 &   3.38 &   uvw2 & 16.42 &  0.06 \\
2455617.54 &   5.81 &   uvw2 & 16.62 &  0.07 \\
2455621.56 &   9.78 &   uvw2 & 16.96 &  0.08 \\
2455632.90 &  20.98 &   uvw2 & 18.47 &  0.17 \\
2455635.07 &  23.12 &   uvw2 & 18.72 &  0.22 \\
2455637.27 &  25.29 &   uvw2 & 18.80 &  0.18 \\
2455640.25 &  28.23 &   uvw2 & 18.40 &  0.17 \\
2455649.14 &  37.01 &   uvw2 & 18.67 &  0.16 \\
2455657.70 &  45.46 &   uvw2 & 18.67 &  0.19 \\
\hline
\multicolumn{2}{l}{$^*$\footnotesize{Rest frame time since $B$-band maximum (2455611.65)}.}
\end{longtable}
}
